Tied-Lora: Enhancing parameter efficiency of LoRA with weight tying

We introduce Tied-LoRA, a novel paradigm leveraging weight tying and selective training to enhance the parameter efficiency of Low-rank Adaptation (LoRA). Our exploration encompasses different plausible combinations of parameter training and freezing, coupled with weight tying, aimed at identifying the optimal trade-off between performance and the count of trainable parameters. Across $5$ diverse tasks and two foundational language models with different parameter counts, our experiments provide comprehensive insights into the inherent trade-offs between efficiency and performance. Our findings reveal a specific Tied-LoRA configuration that distinguishes itself by showcasing comparable performance to LoRA across multiple tasks while utilizing only a fraction of the parameters employed by the standard LoRA method, particularly at elevated ranks. This underscores the efficacy of Tied-LoRA in achieving impressive results with significantly reduced model complexity.

==> avgplot.tex <==

\pgfplotsset{ 
cycle list={%
{draw=black,mark=star,solid},
{draw=black, mark=square,solid}}}

        \definecolor{loracolor}{HTML}{66c2a5}
        \definecolor{tabcolor}{HTML}{fc8d62}
        \definecolor{tuvcolor}{HTML}{8da0cb}
        \definecolor{tacolor}{HTML}{e78ac3}
        \definecolor{tbcolor}{HTML}{e5c494}
	\begin{figure}
	    \centering

	    \subcaptionbox{7B Base Model}
    [\columnwidth]{
        %%%%%%%%%%%iwslt2017,2B%%%%%%%%%%%%%
	\begin{tikzpicture}[font=\tiny]
	    \begin{axis}[
                thin,
		height=0.5\columnwidth,
		width=\columnwidth,
                ylabel style={align=center},
		%ylabel=iwslt2017\\BLEU,
                %ymin=50.06,
		xmode=log,
		log basis y=2,
		log basis x=2,
		xtick={2,4,8,16,32,64,128}]
\addplot[mark=asterisk,loracolor]	coordinates	{	(2,58.05)	(4,58.33)	(8,58.64)	(16,58.61)	(32,57.98)	(64,58.53)	(128,58.43)	};
\addplot[mark=*,tuvcolor]	coordinates	{	(2,56.75)	(4,56.76)	(8,56.44)	(16,57.2)	(32,56.65)	(64,56.51)	(128,55.38)	};
\addplot[mark=square*,tacolor] 	coordinates	{	(2,57.01)	(4,56.9)	(8,56.63)	(16,57.44)	(32,56.45)	(64,56.26)	(128,55.52)	};
\addplot[mark=*,tacolor]	coordinates	{	(2,57.02)	(4,56.57)	(8,56.79)	(16,57.16)	(32,56.6)	(64,56.55)	(128,55.66)	};
\addplot[mark=square*,tabcolor]	coordinates	{	(2,55.59)	(4,56.66)	(8,57.53)	(16,57.53)	(32,57.47)	(64,57.39)	(128,55.53)	};
\addplot[mark=*,tabcolor]	coordinates	{	(2,57.23)	(4,57.91)	(8,57.8)	(16,57.52)	(32,57.93)	(64,58.33)	(128,57.86)	};
\addplot[mark=square*,tbcolor]	coordinates	{	(2,54.93)	(4,56.16)	(8,55.85)	(16,56.06)	(32,55.09)	(64,43.27)	(128,28.02)	};
\addplot[mark=*,tbcolor]	coordinates	{	(2,54.79)	(4,56.0)	(8,56.48)	(16,56.44)	(32,54.9)	(64,40.76)	(128,29.0)	};
	    \end{axis}
	\end{tikzpicture}
    }
    
    \subcaptionbox{2B Base Model}
    [\columnwidth]{
        %%%%%%%%%%%iwslt2017,7B%%%%%%%%%%%%%
	\begin{tikzpicture}[font=\tiny]
	    \begin{axis}[
                thin,
		height=0.5\columnwidth,
		width=\columnwidth,
                ylabel style={align=center},
		%ylabel=iwslt2017\\BLEU,
                %ymin=38.821,
		xmode=log,
		log basis y=2,
		log basis x=2,
		xtick={2,4,8,16,32,64,128}]
\addplot[mark=asterisk,loracolor]	coordinates	{	(2,50.29)	(4,50.68)	(8,51.41)	(16,51.18)	(32,51.16)	(64,51.71)	(128,51.22)	};
\addplot[mark=*,tuvcolor]	coordinates	{	(2,49.92)	(4,49.61)	(8,49.23)	(16,49.05)	(32,47.99)	(64,47.21)	(128,45.6)	};
\addplot[mark=square*,tacolor] 	coordinates	{	(2,49.79)	(4,50.19)	(8,49.51)	(16,49.06)	(32,48.26)	(64,47.52)	(128,45.98)	};
\addplot[mark=*,tacolor]	coordinates	{	(2,49.99)	(4,50.15)	(8,49.77)	(16,49.09)	(32,48.19)	(64,47.72)	(128,46.0)	};
\addplot[mark=square*,tabcolor]	coordinates	{	(2,47.81)	(4,49.2)	(8,49.63)	(16,49.79)	(32,49.86)	(64,49.52)	(128,44.24)	};
\addplot[mark=*,tabcolor]	coordinates	{	(2,50.25)	(4,50.49)	(8,50.77)	(16,50.9)	(32,50.73)	(64,51.11)	(128,50.95)	};
\addplot[mark=square*,tbcolor]	coordinates	{	(2,46.55)	(4,48.23)	(8,47.52)	(16,48.48)	(32,46.86)	(64,35.54)	(128,31.41)	};
\addplot[mark=*,tbcolor]	coordinates	{	(2,47.35)	(4,47.97)	(8,48.32)	(16,48.02)	(32,46.68)	(64,36.13)	(128,31.94)	};
	    \end{axis}
	\end{tikzpicture}
    }
     \subcaptionbox*{}
    [\columnwidth]{
    \begin{tikzpicture}[font=\tiny]
\begin{customlegend}[legend columns=2,legend style={align=left,draw=none,column sep=1ex},
        legend entries={\small{\lora},
                        \small{\Tuv},
                        \small{\TA},
                        \small{\TAuv},
                        \small{\TAB},
                        \small{\TABuv},
                        \small{\TB},
                        \small{\TBu},
                        }]
        \addlegendimage{opacity=0.8,very thick,mark=asterisk,loracolor}
        \addlegendimage{opacity=0.8,very thick,mark=*,tuvcolor}  
        \addlegendimage{opacity=0.8,very thick,mark=square*,tacolor}
        \addlegendimage{opacity=0.8,very thick,mark=*,tacolor}
        \addlegendimage{opacity=0.8,very thick,mark=square*,tabcolor}
        \addlegendimage{opacity=0.8,very thick,mark=*,tabcolor}
        \addlegendimage{opacity=0.8,very thick,mark=square*,tbcolor}
        \addlegendimage{opacity=0.8,very thick,mark=*,tbcolor}
        \end{customlegend}
\end{tikzpicture}
}
	    \caption{Plots showing the performance of the two of the best \tiedlora configurations, (\TAB and \TABuv) along with the baselines \Lora and \Tuv. These show the average score over all $5$ tasks per rank.}
     %https://tex.stackexchange.com/questions/315987/understanding-how-to-have-one-legend-for-a-group-plot
	    \label{fig:plotsall}
	\end{figure}
	


==> layers.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\centering
\small{\resizebox{\columnwidth}{!}{%
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{tabular}{@{}lrrrrr@{}}
\toprule
 & \multicolumn{1}{c}{DialogSum} & \multicolumn{1}{c}{GSM8K} & \multicolumn{1}{c}{HellaSwag} & \multicolumn{1}{c}{Iwslt 2017} & \multicolumn{1}{c}{Squad} \\ \midrule
LoRA Layer 1  & 37.856 & 13.798 & 77.644 & 38.048 & 85.326 \\
LoRA Layer 32 & 31.688 & 2.729  & 47.301 & 22.465 & 56.216 \\
\TAB           & 39.731 & 27.066 & 91.755 & 41.37  & 87.739 \\
\TABuv          & 39.713 & 28.658 & 91.147 & 40.015 & 88.042 \\ \bottomrule
\end{tabular}
}}
\caption{layer vs tied}
\label{tab:layercheck}
\end{table}

==> summary.tex <==
% Please add the following required packages to your document preamble:
\definecolor{gold}{rgb}{1.0, 0.84, 0.0}
\definecolor{palesilver}{rgb}{0.79, 0.75, 0.73}
\definecolor{bronze}{rgb}{0.4, 0.26, 0.13}
\newcommand{\fst}[0]{\textcolor{gold}{$\CIRCLE$}}
\newcommand{\scd}[0]{\textcolor{palesilver}{$\CIRCLE$}}
\newcommand{\trd}[0]{\textcolor{bronze}{$\CIRCLE$}}
\begin{table*}[]
\centering
\small{
%\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}llllll@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Base\\ Model\end{tabular}} & \multirow{2}{*}{Method} & \multicolumn{4}{l}{Avg. Score over tasks @ Rank $r$} \\ \cmidrule(l){3-6} 
                    &       & 2     & 8     & 32    & 128   \\ \midrule
\multirow{8}{*}{2B} & \lora  & 50.29~(100)\fst  & 51.41~(100)\fst  & 51.16~(100)\fst & 51.22~(100)\fst \\ \cmidrule(l){2-6} 
                    & \TABuv & 50.25~(41.7)\scd & 50.77~(13.6)\scd & 50.73~(6.5)\scd & 50.95~(4.8)\scd \\
                    & \TAB   & 47.80~(4.2)      & 49.59~(4.2)      & 49.86~(4.2)     & 44.24~(4.2) \\
                    & \TBu   & 47.35~(3.1)      & 48.32~(3.1)      & 46.68~(3.1)     & 31.94~(3.1) \\ 
                    & \TB    & 46.55~(3.1)      & 47.52~(3.1)      & 46.86~(3.1)     & 31.41~(3.1)\\
                    & \TAuv  & 49.99~(38.6)\trd & 49.77~(10.4)\trd & 48.19~(3.4)     & 46.00~(1.6)\trd  \\
                    & \TA    & 49.79~(1.0)      & 49.51~(1.0)      & 48.26~(1.0)\trd & 45.98~(1.0)\\
                    & \Tuv   & 49.92~(37.5)     & 49.23~(9.4)      & 47.99~(2.4)     & 45.60~(0.6)\\ \midrule
\multirow{8}{*}{7B} & \lora  & 58.05~(100)\fst  & 58.64~(100)\fst  & 57.98~(100)\fst & 58.43~(100)\fst \\ \cmidrule(l){2-6} 
                    & \TABuv & 57.23~(40.6)\scd & 57.80~(12.5)\scd & 57.93~(5.5)\scd & 57.86~(3.7)\scd \\
                    & \TAB   & 55.59~(3.1)      & 57.53~(3.1)\trd  & 57.47~(3.1)\trd & 55.53~(3.1) \\
                    & \TBu   & 54.79~(2.3)      & 56.48~(2.3)      & 54.90~(2.3)     & 29.00~(3.3)  \\ 
                    & \TB    & 54.93~(2.3)      & 55.85~(2.3)      & 55.09~(2.3)     & 28.02~(2.3) \\
                    & \TAuv  & 57.02~(38.3)\trd & 56.79~(10.2)     & 56.60~(3.1)     & 55.66~(1.4)\trd \\
                    & \TA    & 57.01~(0.8)      & 56.63~(0.8)      & 56.45~(0.8)     & 55.52~(0.8) \\
                    & \Tuv   & 56.75~(37.5)     & 56.44~(9.4)      & 56.65~(2.3)     & 55.38~(0.6)\\ \bottomrule
\end{tabular}
%}
}
\caption{Average scores across all tasks at each low rank value for the \tiedlora~methods in comparison with LoRA. The fraction of trainable parameters used by each method compared to \Lora is show in brackets. We indicate the first, second and third highest scoring method for each low-rank setting with \fst, \scd and \trd, respectively.}
\label{tab:summaryscores}
\end{table*}

==> table2b.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[]
\centering
\small{
%\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}llrrrrr@{}}
\toprule
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Base Model\end{tabular}} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Method\end{tabular}} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Dialogsum\\ (RougeL)\end{tabular}} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}GSM8K\\ (Exact Match)\end{tabular}} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}HellaSwag\\ (Acc.)\end{tabular}} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}IWSLT 2017\\ (BLEU)\end{tabular}} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Squad\\ (Exact Match)\end{tabular}} \\ \midrule
\multirow{15}{*}{2B} & \lora       & 38.59(4)  & 12.28(64) & 85.64(64) & 40.19(128) & 83.58(32) \\ \cmidrule(l){2-6} 
& \Tuv        & 37.02(4)  & 6.97(64)  & 75.94(64) & 38.20(128) & 79.43(32) \\
& \TA         & 37.11(4)  & 8.26(64)  & 76.32(64) & 38.12(128) & 79.26(32) \\
& \TAuv       & 37.00(4)  & 8.11(64)  & 77.02(64) & 38.17(128) & 79.50(32) \\
& \TB         & 36.50(4)  & 5.69(64)  & 25.05(64) & 36.46(128) & 76.96(32) \\
& \TBu        & 36.82(4)  & 6.82(64)  & 25.05(64) & 32.98(128) & 77.47(32) \\
& \TAB        & 37.17(4)  & 8.34(64)  & 82.25(64) & 38.58(128) & 81.43(32) \\
& \TABuv      & 37.63(4)  & 9.78(64)  & 85.02(64) & 39.74(128) & 83.02(32) \\ \cmidrule(l){2-6} 
& \Tuv   & 37.28(8)  & 8.26(2)   & 83.41(2)  & 39.15(2)   & 81.77(2)  \\
& \TA    & 37.22(8)  & 9.55(4)   & 83.54(4)  & 39.09(2)   & 82.20(2)  \\
& \TAuv  & 37.29(8)  & 9.40(4)   & 83.64(2)  & 39.11(2)   & 82.41(4)  \\
& \TB    & 37.18(16) & 6.97(8)   & 80.66(4)  & 38.25(4)   & 80.96(4)  \\
& \TBu   & 36.88(32) & 7.20(32)  & 80.51(4)  & 38.30(8)   & 81.03(8)  \\
& \TAB   & 37.55(8)  & 9.40(128) & 83.71(32) & 39.20(64)  & 82.74(16) \\
& \TABuv & 37.81(32) & 10.31(16) & 85.13(32) & 39.74(128) & 83.56(64) \\ \bottomrule
\end{tabular}
}
\caption{Results for 2B base model.}
\label{tab:2bresults}
\end{table*}
